Dataset Condensation via Generative Model

Dataset condensation aims to condense a large dataset with a lot of training samples into a small set. Previous methods usually condense the dataset into the pixels format. However, it suffers from slow optimization speed and large number of parameters to be optimized. When increasing image resolutions and classes, the number of learnable parameters grows accordingly, prohibiting condensation methods from scaling up to large datasets with diverse classes. Moreover, the relations among condensed samples have been neglected and hence the feature distribution of condensed samples is often not diverse. To solve these problems, we propose to condense the dataset into another format, a generative model. Such a novel format allows for the condensation of large datasets because the size of the generative model remains relatively stable as the number of classes or image resolution increases. Furthermore, an intra-class and an inter-class loss are proposed to model the relation of condensed samples. Intra-class loss aims to create more diverse samples for each class by pushing each sample away from the others of the same class. Meanwhile, inter-class loss increases the discriminability of samples by widening the gap between the centers of different classes. Extensive comparisons with state-of-the-art methods and our ablation studies confirm the effectiveness of our method and its individual component. To our best knowledge, we are the first to successfully conduct condensation on ImageNet-1k.

==> tabs/ab_class_embedding.tex <==
\begin{table}[]
\centering
\setlength{\tabcolsep}{6pt}
\begin{tabular}{llll}
\hline
\hline
               & CIFA-10 & CIFA-100 & IN-Sub \\
               \hline
one-hot        & 62.2    &38.1&     20.5  \\
online feature & 64.0    &     39.9    &  22.1      \\
class feature  & 66.2    &    41.9      &  26.6  \\   \hline\hline
\end{tabular}
 \caption{Ablation study on different class conditions.}
  \label{tab:class}
\end{table}

==> tabs/ab_image_scaleup.tex <==
\begin{table}[t]
\centering
\resizebox{0.45\textwidth}{!}{

\begin{tabular}{c|cc}
\hline
  \diagbox{Resolution}{ Classes}  & 500   & 1000    \\
  \hline
64  & 33.9 \vs 61.4 & 34.6 \vs 122.9 \\
128 & 34.4 \vs 245.6 & 35.0 \vs 491.6 \\
256 & 39.5 \vs 982.4& 40.1 \vs 1966.4 \\
\hline
\end{tabular}}
\caption{Number of parameter(MB)  comparisons between our generative model and pixels format with number of classes. 10 images per class(ours \vs pixel format).}
\label{para1}
\end{table}

% \begin{table}[h]
% \centering
% \resizebox{0.45\textwidth}{!}{

% % \begin{tabular}{c|cc}
% % \hline
% %   \diagbox{Resolution}{Number of Classes}  & 500   & 1000  \\
% %   \hline
% % 64  & 61.4 & 122.9 \\
% % 128 & 245.6 & 491.6  \\
% % 256 & 982.4& 1966.4 \\
% % \hline
% % \end{tabular}}
% % \caption{Number of parameter(MB) of pixel format with number of classes. 10 images per class.}
% % \label{pixel_cl}
% % \end{table}


\begin{table}[t]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{c|ccc}


\hline
  \diagbox{Res.}{IPC}  & 10   & 50   & 100  \\
  \hline
64  & 34.6 \vs 122.9 & 39.7 \vs 614.5& 46.1 \vs 1229\\
128 & 35.0 \vs 491.6 & 40.1 \vs 2458 & 46.5 \vs 4916 \\
256 & 40.1 \vs 1966.4 & 45.2 \vs 9832 & 51.6 \vs 19664\\
\hline
\end{tabular}}
\caption{Number of parameter(MB)  comparisons between our generative model and pixels format with images per Class. 1000 classes (ours \vs pixel format).}
\label{para2}
\end{table}

% \begin{table}[h]
% \centering
% \resizebox{0.45\textwidth}{!}{
% \begin{tabular}{c|ccc}
% \hline

%   \diagbox{Resolution}{IPC}  & 10   & 50   & 100  \\
%   \hline
% 64  & 122.9 & 614.5 & 1229 \\
% 128 & 491.6 & 2458 & 4916 \\
% 256 & 1966.4 & 9832 & 19664\\
% \hline
% \end{tabular}}
% \caption{Number of parameter (MB) of pixel format with images per class. 1000 classes.}
% \label{pixel}
% \end{table}

==> tabs/ab_network_for_distilled.tex <==
\begin{table}[h]
\centering
\begin{tabular}{llll}
\hline
         & Fixed & Random & Subset \\
         \hline
accuracy & 63.4  & 65.0  & 66.2\\ 
\hline
\end{tabular}
\caption{Ablation on different association types. The results are for 10 images per class setting on CIFAR-10.}
\label{hhd}
\end{table}

==> tabs/ab_z_code.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]

\setlength{\tabcolsep}{2pt}
    \centering
	\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{l|lll}
\hline\hline

                                                            & CIFA-10 & CIFA-100 & IN-Sub \\
                                  \hline
uniform sample                                          & 55.3    &      27.1    & 12.2  \\
\hline
random with threshold                                                       & 55.9    &   28.4       & 12.5   \\
\hline
           

          learnable codebooks                          & 66.2    &     41.9     & 26.6 \\
                                 \hline\hline
\end{tabular}}
\caption{Ablation study on different input samples}
\label{code}
\end{table}

==> tabs/pretrained_weight.tex <==
\begin{table}[!h]
  \centering

\begin{tabular}{l|cc}
\hline
                 & CIFRA-10 & CIFRA-100 \\
                 \hline
with pretraining & 66.2     & 41.9      \\
w/o pretraining  & 63.2     & 36.6    \\ 
\hline
\end{tabular}

  \caption{Ablation study on generator pretraining.}
  \label{tab:pre}
\end{table}

==> tabs/sup_sota.tex <==
\begin{table}[t]
 
	\begin{center}
	      \setlength{\tabcolsep}{0.5pt}
        \resizebox{1\columnwidth}{!}{
		\begin{tabular}{c|cc|cc|cc}
			\toprule
			  Dataset &  \multicolumn{2}{c|}{SVHN} &  \multicolumn{2}{c|}{CIFAR10} & \multicolumn{2}{c}{CIFAR100}  \\
			  Store-IPC &  10 & 50 & 10 & 50 & 10 & 50  \\
			
			\hline
		
	
			
		HaBa\cite{liu2022dataset}

			& 83.2\tiny$\pm$0.3
			& 88.3\tiny$\pm$0.1
			& 69.9\tiny$\pm$0.4
			& 74.0\tiny$\pm$0.2
			& 40.2\tiny$\pm$0.2
   	     & 46.1\tiny$\pm$0.2

  \\
			IDC\cite{data-para}
			& 87.3\tiny$\pm$0.2
			& 90.2\tiny$\pm$0.1
			& 67.5\tiny$\pm$0.5
			& 74.5\tiny$\pm$0.1
			& 44.8\tiny$\pm$0.2
   	     	& -


               \\

               Rem.\cite{remember}
			& 89.1\tiny$\pm$0.2
			& 89.5\tiny$\pm$0.2
			& 71.2\tiny$\pm$0.4
			& 73.6\tiny$\pm$0.5
			& 42.9\tiny$\pm$0.2
   	      & -
		
			\\
			\textbf{Ours}
			& \textbf{91.6\tiny$\pm$0.3}
			& \textbf{93.0\tiny$\pm$0.1}
			& \textbf{71.8\tiny$\pm$0.2}
			& \textbf{74.9\tiny$\pm$0.1}
			& \textbf{49.6\tiny$\pm$0.1}
                & \textbf{51.5\tiny$\pm$0.1}
	 \\
			\hline
			Full dataset
			& \multicolumn{2}{c}{95.4\tiny$\pm$0.1} 
			& \multicolumn{2}{c}{84.8\tiny$\pm$0.1} 
			& \multicolumn{2}{c}{56.2\tiny$\pm$0.3}
			\\
			\bottomrule
		\end{tabular}
		}
  \caption{\small \textbf{SOTA Comparisons under memory story budget.}} \label{sota2}
	\end{center}
	\small
	\vspace{-0.25in}
\end{table}
